Full version: An evaluation of estimation techniques for probabilistic reachability

We evaluate numerically-precise Monte Carlo (MC), Quasi-Monte Carlo (QMC) and Randomised Quasi-Monte Carlo (RQMC) methods for computing probabilistic reachability in hybrid systems with random parameters. Computing reachability probability amounts to computing (multidimensional) integrals. In particular, we pay attention to QMC methods due to their theoretical benefits in convergence speed with respect to the MC method. The Koksma-Hlawka inequality is a standard result that bounds the approximation of an integral by QMC techniques. However, it is not useful in practice because it depends on the variation of the integrand function, which is in general difficult to compute. The question arises whether it is possible to apply statistical or empirical methods for estimating the approximation error. In this paper we compare a number of interval estimation techniques based on the Central Limit Theorem (CLT), and we also introduce a new approach based on the CLT for computing confidence intervals for probability near the borders of the [0,1] interval. Based on our analysis, we provide justification for the use of the developed approach and suggest usage guidelines for probability estimation techniques.

==> Section5-ToolsModels.tex <==
\section{Bounded Reachability calculation tools and testing models}

\subsection{Software}
%\paragraph{ProbReach.}
We conducted our research on the basis of ProbReach tool \cite{ProbReach} for computing bounded reachability in stochastic parametric hybrid systems (SPHS). ProbReach can use either d$Real$ \cite{dreal} or $iSat-ODE$ \cite{DBLP:conf/mbmv/ScheiblerKB13} solvers for analyzing (standard) bounded reachability question. %$dReal$ solves expression that can be encoded as first-order logic formulas over the real numbers.

Essentially, both d$Real$ and $iSat-ODE$ are implementations of a $\delta$-complete decision procedure for first-order logic functions over the reals that may include nonlinear functions and ordinary differentiation equations (ODEs).

%It executes publicity available libraries and can be downloaded from //link to github.

%ProbReach aims to encode PHS and SPSH by using probabilistic delta-reachability format (PDRF), which extends delta-reachability format introduced in dReach [?]. ProbReach involves PSH parser translator, that is applied to transform the input model specified in PDRF into program acceptable representation. The full information about PHS format can be found in [?]. We used d$Real$ solver within the ProbReach tool to conduct our research.

%The last version of ProbrReach supports two solvers - d$Real$ and $iSat-ODE$. 

%\paragraph{DReal solver.}
%http://dreal.github.io/
%dReal solves expression that can be encoded as first-order logic formulas over the real numbers. %It can be applied to the broad range of nonlinear real functions. dReal is based on the $\delta$-complete decision procedure, which returns $unsat$ or $sat$ results according to input formulas and specified $\delta$. It also supports ODEs. More technical information about dReal tool implementation can be found in [?].



%\paragraph{ solver.}
%http://www.avacs.org/tools/isatode/
%iSAT-ODE solves arithmetic constraint systems containing ODEs. It focuses on the formulae that originate from the predicative encoding of bounded model controlling the characteristics of hybrid discrete-continuous systems. The continuous dynamics of such systems can be shown by ODEs. The main function of iSAT-ODE solver within ProbReach implementation is unrolling the reachability formula. More technical iSAT-ODE tool documentation can be found in [].

\subsection{Testing models}
The main aim of the tests conducted is to reveal how different model types and their complexity can affect the computational result. Five models were chosen for our experiments. %Input parameters of the verified models obtained via ProbReach for confidence interval computation and the error estimation are presented in Table 1.
%The results of computation for different estimation methods are presented in Table 1. 
    
\paragraph{ ``Good'' and ``Bad'' models.}
These models represent single mode non-hybrid systems with constant flow dynamics. Initially, both systems have a state defined by the predicate $(x(0)=r)\wedge (n\in [0,1])$, where $n$ is a  parameter on $[0,1]$ and $r$ is uniformly distributed over [0,1]. The probability function in the \say{Good} model case is constant $p(n)=0.1$, while in the \say{Bad} model case it is equal to $p(n)=4n^2-4n+1$, which reaches its minimum value of 0 at $n=0.5$ and the maximum value of 1 at $n=0$  and $n=1$.
ProbReach is used to compute 0-step bounded reachability probability for the \say{Good} model goal specified by the predicate $(x\leq 0.9n+0.1) \wedge (x \geq 0.9n)$ and for the \say{Bad} model goal specified by the predicate $(x\leq 2(n+0.5)^2+0.5) \wedge (x \geq -2(n-0.5)^2+0.5).$

\paragraph{Deceleration model.}
%This model represents a car deceleration scenario. ProbReach is used to compute the probability of a car stopping within 400 meters. During the first mode the car accelerates from 0 to 100 km/h and its velocity changes as $v^{\prime}(t)=\alpha \exp^{-\alpha t +\beta}-c_d v^2(t)$, where $\alpha=0.05776$, $\beta \sim N(4,0.1)$ and $c_d=3.028 \cdot 10-4m^{-1}$ is the drag coefficient. During the second mode driver is reacting within 1.2 seconds and starting deceleration according to the velocity equation $v^{\prime}(t)=-c_d v^2(t)$. The final mode presents car deceleration. The distance for deceleration $s(t)$ is obtained by $s^\prime (t)=v(t)$ equation.  
This hybrid model represents a car deceleration scenario. During the first mode the car accelerates from 0 to 100 km/h, using a nonlinear function that depends on random parameter. During the second mode driver is reacting after 1.2 seconds and starting deceleration. The final mode presents car deceleration. The model takes into account that velocity changes due to friction. ProbReach is used to compute the probability of a car stopping within 400 meters. 

\paragraph{Collision model.}
%This model represents two cars collision scenario with initial speed 11.12 $m/sec$. Car1 and Car2 move on the same track, starting at $s_1(0)=0$ and $s_2(0)=v_1$. During the first mode Car2 continues movement with speed $v_2$. Car1 changes track and starts accelerating at $a_{a1}=3$ $m/sec^2$ until it gets ahead of Car2 by safely distance $v_2\cdot t_{safe}$. During the second mode Car2 returns to the initial track and starts decelerating at $a_{d1} \sim N(-2.0,0.2)$ $m/sec^2$, while Car2 driver is taking time to react and then starting deceleration with acceleration $a_{d2} \sim N(-0.5,0.1)$ $m/sec^2$. We used three different configurations of this model: $basic$ model contains one random parameters; $extended$ and $advanced$ models contain two random parameters.
This hybrid model represents a two car collision scenario. Car1 and Car2 move on the same lane with speed 11.12 $m/sec$. During the first mode Car2 continues movement, while Car1 changes lane and starts accelerating until it gets ahead of Car2 by a safe distance. During the second mode Car2 returns to the initial lane and starts decelerating, while Car2's driver takes time to react and then starts deceleration. ProbReach is used to compute the probability of the cars colliding for three different configurations of this model: the $basic$ model contains one random parameter - deceleration of Car1 ; $extended$ and $advanced$ models contains two random parameters for the deceleration of Car1 and Car2.

\paragraph{Anesthesia model.}
%The Anesthesia model presents anesthesia deliverywhile drug concentration changes with metabolic process in the body. ProbReach computes the probability of reaching unsafe state $(c_p(t)\geq 6) \vee (c_p(t) \leq 1) \vee (c_1(t)\geq 10) \vee(c_1(t) \leq0) \vee(c_2(t)\geq 10) \vee (c_2(t) \leq 0)$ in 3 jumps within 60 minutes, starting at time 0 and having drug infusion rate with changes, where $c_p$ - plasma drug concentration, $c_1$- fast peripheral compartment drug concentration and $c_2$ - slow peripheral compartment drug concentration.
This model represents anesthesia delivery. It tracks the drug concentration which changes as the result of metabolic processes in human body. The model's scenario assumes that drug delivery is continuous, but every 15 minutes (starting at time 0) the drug infusion rate is subject to random errors. ProbReach computes the probability of reaching the unsafe state $(c_p(t)\geq 6) \vee (c_p(t) \leq 1) \vee (c_1(t)\geq 10) \vee(c_1(t) \leq0) \vee(c_2(t)\geq 10) \vee (c_2(t) \leq 0)$ in 3 jumps within 60 minutes, where $c_p$ - plasma drug concentration, $c_1$- fast peripheral compartment drug concentration and $c_2$ - slow peripheral compartment drug concentration.    % according to the plasma drug concentration, fast peripheral compartment drug concentration and  slow peripheral compartment drug concentration.
$$
$$
More information about the models can be found in the thesis, written by Fedor Shmarov (Newcastle University).

